Some observations on the logical foundations of inductive theorem proving

In this paper we study the logical foundations of automated inductive theorem proving. To that aim we first develop a theoretical model that is centered around the difficulty of finding induction axioms which are sufficient for proving a goal. Based on this model, we then analyze the following aspects: the choice of a proof shape, the choice of an induction rule and the language of the induction formula. In particular, using model-theoretic techniques, we clarify the relationship between notions of inductiveness that have been considered in the literature on automated inductive theorem proving. This is a corrected version of the paper arXiv:1704.01930v5 published originally on Nov.~16, 2017.

==> macros.tex <==
\makeatletter

\theoremstyle{plain}\newtheorem*{compobs}{Computational Observation}

%\theoremstyle{definition}
%\newtheorem*{defn}{Definition}
%\newtheorem*{compobs}{Computational Observation}
%\newtheorem{thm}{Theorem}[section]
%\newtheorem{eg}[thm]{Example}
%\newtheorem{lem}[thm]{Lemma}
%\newtheorem{prop}[thm]{Proposition}
%\newtheorem{cor}[thm]{Corollary}
%\newtheorem{qn}[thm]{Question}
%\theoremstyle{remark}
%\newtheorem{rmk}[thm]{Remark}

\newcommand{\cprob}[3]{
\begin{center}
\fbox{
  \parbox{120mm}{
    {\centering {#1}\par}\parskip=1ex
    \begin{tabular}{rl}
      {\bf Input:} & \parbox{95mm}{#2}\\[0.5mm]
      {\bf Output:} & \parbox[t]{95mm}{#3}
    \end{tabular}
  }
}
\end{center}
}

\let\phi\varphi
\let\leq\leqslant
\let\geq\geqslant
\renewcommand{\theequation}{\fnsymbol{equation}}

\let\partref\eqref
\let\itemref\eqref
\let\fmaref\eqref
\let\condref\eqref
\let\axref\ref

\newcommand{\mar}[1]{\marginpar{\raggedright#1}}
\newcommand{\defm}[1]{\emph{#1}}
\newcommand{\mathnoun}[1]{\mathrm{#1}}
\newcommand{\qequals}{\quad=\quad}
\newcommand{\qand}{\quad\text{and}\quad}

\newcommand{\tfaeenum}
 {\renewcommand{\theenumi}{\roman{enumi}}%
  \renewcommand{\labelenumi}{(\theenumi)}}
\newcommand{\propenum}
 {\renewcommand{\labelenumi}{(\theenumi)}}
\newcommand{\partenum}
 {\renewcommand{\theenumi}{\alph{enumi}}%
  \renewcommand{\labelenumi}{(\theenumi)}}

\newlength\@templen
\newcommand{\SpaceIfNZerowd}[1]{%
 \settowidth{\@templen}{$#1$}
 \ifdim\@templen>0pt \ \fi{#1}}
\let\SpaceXIfNZerowd\SpaceIfNZerowd
\newcommand{\fa}[2]{\forall{#1}\SpaceXIfNZerowd{#2}}
\newcommand{\ex}[2]{\exists{#1}\SpaceXIfNZerowd{#2}}
\newcommand{\falt}[3]{\forall{#1{<}{#2}}\SpaceIfNZerowd{#3}}
\newcommand{\exlt}[3]{\exists{#1{<}{#2}}\SpaceIfNZerowd{#3}}
\newcommand{\fale}[3]{\forall{#1{\leq}{#2}}\SpaceIfNZerowd{#3}}
\newcommand{\exle}[3]{\exists{#1{\leq}{#2}}\SpaceIfNZerowd{#3}}
\newcommand{\fage}[3]{\forall{#1{\geq}#2}\SpaceIfNZerowd{#3}}
\newcommand{\exge}[3]{\exists{#1{\geq}#2}\SpaceIfNZerowd{#3}}
\newcommand{\exi}[1]{\ex{{!}#1}}

\newcommand{\IN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\proves}{\vdash}
\newcommand{\nproves}{\nvdash}
\newcommand{\isprovedby}{\dashv}
\newcommand{\then}{\rightarrow}
\newcommand{\Then}{\Rightarrow}
\newcommand{\nsc}{\leftrightarrow}
\newcommand{\Nsc}{\Leftrightarrow}
\newcommand{\rel}[1]{^{#1}}
\newcommand{\setm}{\setminus}
\DeclareMathOperator*{\bigwwedge}
 {\mathchoice{\bigwedge\mkern-16.5mu\bigwedge}
             {\bigwedge\mkern-12mu\bigwedge}
             {\bigwedge\mkern-13mu\bigwedge}
             {\bigwedge\mkern-11mu\bigwedge}}
\DeclareMathOperator*{\bigvvee}
 {\mathchoice{\bigvee\mkern-16.5mu\bigvee}
             {\bigvee\mkern-12mu\bigvee}
             {\bigvee\mkern-13mu\bigvee}
             {\bigvee\mkern-11mu\bigvee}}

\newcommand{\BA}{\mathscr{B}}
\newcommand{\lang}{\mathscr{L}}
\newcommand{\Lor}{\lang_{\mathnoun{OR}}}
\newcommand{\Lr}{\lang_{\mathnoun R}}
\newcommand{\ind}{\mathnoun{I}}
\newcommand{\lnp}{\mathnoun{L}}
\newcommand{\PA}{\mathnoun{PA}}
\newcommand{\ACAnaught}{\mathnoun{ACA}_0}
\newcommand{\Ztwo}{\mathnoun{Z}_2}
\newcommand{\PAminus}{\mathord{\mathrel{\PA}\joinrel\mathrel{\mbox{\vphantom{$\PA$}}^{\mathord-}}}}
\newcommand{\IOpen}{\ind\mathnoun{Open}}
\newcommand{\ISigma}{\ind\Sigma} % for \ISigma_k
\newcommand{\LOpen}{\lnp\mathnoun{Open}}
\newcommand{\LK}{\mbox{\rm LK}} % the sequent calculus LK
\newcommand{\seq}{\longrightarrow} % the sequent sign
\newcommand{\Con}{\mbox{\rm Con}} % consistency of ...
\newcommand{\Ind}{\mbox{\rm Ind}} % induction rule (for the sequent calculus)
\newcommand{\p}{\mbox{\rm p}\nobreakdash}% for \p-inductive

\newcommand{\ITP}{\textsc{ITP}}
\newcommand{\ITPEq}{\ensuremath{\textsc{ITP}_\textsc{Eq}}}
\newcommand{\ITPU}{\ensuremath{\textsc{ITP}_\textsc{U}}}
\newcommand{\ITPOpen}{\textsc{ITPOpen}}
\newcommand{\ITPOpenLR}{\ensuremath{\textsc{ITPOpen}(\Lr)}}
\newcommand{\BAITP}{\ensuremath{\BA}\ITP}
\newcommand{\BAxITP}{\ensuremath{\BA(x)}\ITP}

\newcommand{\newX}{\mathsf{X}}
\makeatother
\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "induction_rules.tex"
%%% End:

